Convergence of Adam Under Relaxed Assumptions

In this paper, we provide a rigorous proof of convergence of the Adaptive Moment Estimate (Adam) algorithm for a wide class of optimization objectives. Despite the popularity and efficiency of the Adam algorithm in training deep neural networks, its theoretical properties are not yet fully understood, and existing convergence proofs require unrealistically strong assumptions, such as globally bounded gradients, to show the convergence to stationary points. In this paper, we show that Adam provably converges to $\epsilon$-stationary points with ${O}(\epsilon^{-4})$ gradient complexity under far more realistic conditions. The key to our analysis is a new proof of boundedness of gradients along the optimization trajectory of Adam, under a generalized smoothness assumption according to which the local smoothness (i.e., Hessian norm when it exists) is bounded by a sub-quadratic function of the gradient norm. Moreover, we propose a variance-reduced version of Adam with an accelerated gradient complexity of ${O}(\epsilon^{-3})$.

==> Sections/proof_adam.tex <==
In this section, we provide proofs of Theorem~\ref{thm:main_rho_2} and \ref{thm:main_rho_1} for convergence of Adam. For completeness, we repeat some important technical definitions here.  First, we define $$\epsilon_t:=\hm_t-\nabla f(x_t)$$ as the deviation of the re-scaled momentum from the actual gradient. We formally define stopping time $\tau$ as
\begin{align*}
\tau := \min\{t\mid \norm{\nabla f(x_t)}>G\}\land (T+1),
\end{align*}
i.e.,  $\tau$ is the first time when the gradient norm is strictly greater than $G$, and if the gradient norm is always bounded by $G$ up to time $T$, we truncate it and set $\tau=T+1$ to make sure it is bounded. It is clear to see that $\tau$ is a stopping time\footnote{Indeed, $\tau-1$ is also a stopping time because $\nabla f(x_t)$ only depends on $\{\xi_s\}_{s<t}$, but that is unnecessary for our analysis.} with respect to  $\{\xi_t\}_{t\ge1}$ because the event $\{\tau\ge t\}$ is a function of $\{\xi_s\}_{s<t}$ and independent of $\{\xi_s\}_{s\ge t}$. Next, let
\begin{align*}
h_t:=\frac{	\eta}{\sqrt{\hv_t}+\lambda}
\end{align*}
be the stepsize vector and $H_t:=\diag(h_t)$ be the diagonal stepsize matrix. Then the update rule can be written as
\begin{align*}
	x_{t+1} = x_t-h_t\cdot \hm_t = x_t-H_t\hm_t.
\end{align*}
Finally, as in Corollary~\ref{cor:l0l1}, we define the following constants.
\begin{align*}
	r:= \frac{(L_0/L_\rho)^{1/\rho}}{3L_0+4L_\rho G^\rho},\quad P:=\frac{1}{2}(3L_0+8L_\rho G^\rho).
\end{align*}

First note that when $t<\tau$, all the quantities in the algorithm are well bounded. In particular, we have the following lemma.
\begin{lemma}
	\label{lem:bounded_everything}
	If $t<\tau$, we have
	\begin{align*}
		\norm{\nabla f(x_t)}\le G, \quad\norm{\nabla f(x_t,\xi_t)}\le G+\sigma,&\quad \norm{\hm_t}\le G+\sigma,\quad \hv_t\preceq (G+\sigma)^2, \quad 
		 \frac{\eta}{G+\sigma+\lambda}	\preceq h_t \preceq \frac{\eta}{\lambda}.
	\end{align*}
\end{lemma}
Combining Lemma~\ref{lem:bounded_everything} and Corollary~\ref{cor:update_bound}, we directly get the following Corollary which bounds each update before $\tau$ by a constant.

\begin{corollary}
	\label{cor:bound_update_before_tau}
	If $t<\tau$ and choosing $G\ge\sigma$, we have 
	\begin{align*}
		\norm{x_{t+1}-x_t}\le \eta D,\text{ where }D :=\left\{
		\begin{array}{lr}
		\min\{\sqrt{d}, 2 G/\lambda\}& \text{if } \beta=\betasq, \\
		2 G/\lambda& \text{otherwise. } 
		\end{array}
		\right.
	\end{align*}
\end{corollary}


Next, we provide a descent lemma for ADAM.
\begin{lemma}
	\label{lem:descent_lemma}
	If $t<\tau$, choosing $G\ge \sigma+\lambda$ and $\eta\le \min\left\{\frac{r}{D},\frac{\lambda}{6P}\right\}$, we have
	\begin{align*}
			f(x_{t+1})-f(x_t) \le& -\frac{\eta}{4G}\norm{\nabla f(x_t)}^2 + \frac{\eta}{\lambda}\norm{\epsilon_t}^2.
	\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lem:descent_lemma}]
	By Lemma~\ref{lem:bounded_everything}, we have if $t<\tau$,
	\begin{align}
	 \frac{\eta I}{2G}\le \frac{\eta I}{G+\sigma+\lambda}	\preceq H_t \preceq \frac{\eta I}{\lambda}.\label{eq:bd2}
	\end{align}
	Since we choose $\eta\le \frac{r}{D}$, by Corollary~\ref{cor:bound_update_before_tau}, we have $\norm{x_{t+1}-x_t}\le r$ if $t<\tau$. Then we can apply Lemma~\ref{lem:l0l1} to show that for any $t<\tau$,
	\begin{align*}
		f(x_{t+1})-f(x_t) \le& {(\nabla f(x_t))^\top}{(x_{t+1}-x_t)} +\frac{1}{2}(L_0+L_\rho \norm{\nabla f(x_t)}^\rho)\norm{x_{t+1}-x_t}^2\\
		=&  -(\nabla f(x_t))^\top H_t \hm_t + \frac{1}{2}(L_0+L_\rho \norm{\nabla f(x_t)}^\rho)\hm_t^\top H_t^2 \hm_t\\
		\le & -\norm{\nabla f(x_t)}_{H_t}^2-(\nabla f(x_t))^\top H_t\epsilon_t +\frac{\eta}{2\lambda}(L_0+L_\rho G^\rho)\norm{\hm_t}_{H_t}^2\\
		\le & -\frac{2}{3}\norm{\nabla f(x_t)}_{H_t}^2 + \frac{3}{4}\norm{\epsilon_t}_{H_t}^2 +\frac{\eta P}{\lambda}\left(\norm{\nabla f(x_t)}_{H_t}^2 + \norm{\epsilon_t}_{H_t}^2\right)\\
		\le& -\frac{1}{2}\norm{\nabla f(x_t)}_{H_t}^2 + \norm{\epsilon_t}_{H_t}^2\\
		\le & -\frac{\eta}{4G}\norm{\nabla f(x_t)}^2 + \frac{\eta}{\lambda}\norm{\epsilon_t}^2.
%		\le& -\norm{\nabla f(x_t)}_{H_t}^2-(\nabla f(x_t))^\top H_t\epsilon_t+\frac{\eta^2 L_0}{2\lambda^2}\norm{\hm_t}^2+\frac{\eta^2\sqrt{d}L_\rho }{2\lambda}\norm{\hm_t}\norm{\nabla f(x_t)}\\
%		\le &-\frac{1}{2}\norm{\nabla f(x_t)}_{H_t}^2 + \frac{1}{2}\norm{\epsilon_t}_{H_t}^2+\frac{\eta^2\sqrt{d}L_\rho }{4\lambda}\norm{\nabla f(x_t)}^2+\eta^2\left(\frac{ L_0}{2\lambda^2}+\frac{\sqrt{d}L_\rho }{4\lambda}\right)\norm{\hm_t}^2\\
%		\le & -\frac{\eta}{4G}\norm{\nabla f(x_t)}^2 + \frac{\eta}{2\lambda}\norm{\epsilon_t}^2+\eta^2\left(\frac{ L_0}{\lambda^2}+\frac{\sqrt{d}L_\rho }{\lambda}\right)\left(\norm{\epsilon_t}^2+\norm{\nabla f(x_t)}^2\right)\\
%		\le& -\frac{\eta}{8G}\norm{\nabla f(x_t)}^2 + \frac{\eta}{\lambda}\norm{\epsilon_t}^2,
	\end{align*}
	where the second inequality is due to $\norm{\nabla f(x_t)}\le G$ if $t<\tau$; the third inequality is due to $\langle a,b\rangle_A\le \frac{1}{3}\norm{a}_A^2+\frac{3}{4}\norm{b}_A^2$ and $\norm{a+b}_A^2\le 2(\norm{a}_A^2+\norm{b}_A^2)$ for any positive definite matrix $A$; the second last inequality uses $\eta\le \frac{\lambda}{6P}$; and the last inequality is due to \eqref{eq:bd2}.
\end{proof}

The following lemma bounds the sum of the error term $\norm{\epsilon_t}^2$ before the stopping time $\tau$. Since its proof is complicated, we defer it in Appendix~\ref{app:proof_lemma_sum_moment_error}.
\begin{lemma}
	\label{lem:sum_moment_error}
	If $G\ge2\sigma$ and $\eta\le \min\left\{\frac{r}{D}, \frac{\lambda^{3/2}\beta}{6P\sqrt{G}},\frac{\sigma \beta}{DP}\right\} $, with probability $1-\delta$,
	\begin{align*}
	\sum_{t=1}^{\tau-1} \norm{\epsilon_{t}}^2 - \frac{\lambda}{8G}\norm{\nabla f(x_{t})}^2 \le 8\sigma^2\left(1/\beta+\beta T\right)+ 20\sigma^2\sqrt{(1/\beta^2+T)\log(2/\delta)} .
	\end{align*}
\end{lemma}

\begin{lemma}
	\label{lem:upper_bound}
	If $G\ge2\max\left\{\lambda,\sigma\right\}$ and $\eta\le \min\left\{\frac{r}{D}, \frac{\lambda^{3/2}\beta}{6P\sqrt{G}},\frac{\sigma \beta}{DP}\right\} $, with probability $1-\delta$,
	\begin{align*}
	\sum_{t=1}^{\tau-1} \norm{\nabla f(x_{t})}^2\le \frac{8G}{\eta\lambda}\left(\Delta_0\lambda+8\sigma^2\left(\eta/\beta+\eta\beta T\right)+20\sigma^2 \eta \sqrt{(1/\beta^2+T)\log(2/\delta)}\right)
	\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lem:upper_bound}]
	By telescoping, Lemma~\ref{lem:descent_lemma} implies
	\begin{align}
	\sum_{t=1}^{\tau-1} 2\norm{\nabla f(x_{t})}^2 -\frac{8G}{\lambda}\norm{\epsilon_{t}}^2\le \frac{8G}{\eta}\left(f(x_1)-f(x_\tau)\right)\le \frac{8\Delta_0G}{\eta}.\label{eq:eq1}
	\end{align}
	Lemma~~\ref{lem:sum_moment_error} could be written as
	\begin{align}
		\sum_{t=1}^{\tau-1} \frac{8G}{\lambda}\norm{\epsilon_{t}}^2-\norm{\nabla f(x_{t})}^2\le \frac{8G}{\lambda}\left(8\sigma^2\left(1/\beta+\beta T\right)+ 20\sigma^2 \sqrt{(1/\beta^2+T)\log(2/\delta)}\right) .\label{eq:eq2}
	\end{align}
	\eqref{eq:eq1} + \eqref{eq:eq2} gives the desired result.
\end{proof}


\begin{lemma}
	\label{lem:lower_bound} Suppose $G\ge 2\max\{\norm{\nabla f(x_1)},\sigma\}$ and $\eta\le\min\left\{\frac{r}{D},\frac{G}{4DP}\right\} $. If $\tau\le T$, i.e., there exists some time up to $T$ when the gradient norm is greater than $G$, the following inequality holds almost surely
	\begin{align*}
	\sum_{t=1}^{\tau-1} \norm{\nabla f(x_t)}^2> \frac{G^3}{16\eta DP}.
	\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lem:lower_bound}]
	If $\tau\le T$, we define $\tau_{1/2}$ as the last time before $\tau$ such that $\norm{\nabla f(x_t)}\le G/2$, i.e.,
	\begin{align*}
	\tau_{1/2} = \max \{t<\tau\mid \norm{\nabla f(x_t)}\le G/2\}.
	\end{align*}
	We know $\tau_{1/2}$ is well defined since we assume $\norm{\nabla f(x_1)}\le G/2$. By the definition of $\tau$ and $\tau_{1/2}$, we know $\norm{\nabla f(x_{\tau})}>G$ and $\norm{\nabla f(x_{\tau_{1/2}})}\le G/2$, which implies
	\begin{align*}
	\frac{G}{2}<&\norm{\nabla f(x_{\tau})-\nabla f(x_{\tau_{1/2}})}\\\le& \sum_{t=\tau_{1/2}}^{\tau-1}\norm{ \nabla f(x_{t+1}) -\nabla f(x_t)  }\\
	\le&\sum_{t=\tau_{1/2}}^{\tau-1} (L_0+L_\rho \norm{\nabla f(x_t)}^\rho)\norm{x_{t+1}-x_t}\\
	\le & \sum_{t=\tau_{1/2}}^{\tau-1} \eta D(L_0+L_\rho G^\rho)\\
	\le& \eta DP(\tau-\tau_{1/2}),
	\end{align*}
	where the third inequality uses Assumption~\ref{ass:l0l1} since $\norm{x_{t+1}-x_t}\le \eta D\le r$ if choosing $\eta\le \frac{r}{D}$; and the fourth inequality uses $\norm{\nabla f(x_t)}\le G$ if $t<\tau$.
	Therefore
	\begin{align*}
		\tau-\tau_{1/2}> \frac{G}{2\eta DP}.
	\end{align*}
	Then we have
	\begin{align*}
	\sum_{t=1}^{\tau-1} \norm{\nabla f(x_t)}^2\ge& \sum_{t=\tau_{1/2}+1}^{\tau-1} \norm{\nabla f(x_t)}^2\ge(\tau-\tau_{1/2}-1)\cdot \frac{G^2}{4}\\
	>&  \frac{G^3}{8\eta DP}-\frac{G^2}{4}\ge \frac{G^3}{16\eta DP},
	\end{align*}
	where the second inequality is due to $\norm{\nabla f(x_t)}\ge G/2$ if $t>\tau_{1/2}$; and the last inequality uses $\eta\le \frac{G}{4 DP}$.

\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:main_rho_2} and Theorem~\ref{thm:main_rho_1}] Here prove Theorem~\ref{thm:main_rho_2} and Theorem~\ref{thm:main_rho_1} together because their only difference is parameter choices.
First, it is straight forward to verify that the parameter choices in both theorems satisfy the requirements of all the lemmas in this paper.
According to Lemma~\ref{lem:upper_bound}, there exists some event $\cE$ with $\Pro(\cE)\ge1-\delta$, such that conditioned on $\cE$, we have
	\begin{align}
\sum_{t=1}^{\tau-1} \norm{\nabla f(x_{t})}^2\le \frac{8G}{\eta\lambda}\left(\Delta_0\lambda+8\sigma^2\left(\frac{\eta}{\beta}+\eta\beta T\right)+20\sigma^2 \eta \sqrt{(1/\beta^2+T)\log(2/\delta)}\right)=: I_1.\label{eq:thm_up}
\end{align}
By Lemma~\ref{lem:lower_bound}, if $\tau\le T$, we have
	\begin{align*}
\sum_{t=1}^{\tau-1} \norm{\nabla f(x_t)}^2> \frac{G^3}{16\eta DP}=:I_2.
\end{align*}
With some standard but messy calculations (see Lemma~\ref{lem:calculations}), we can show $I_1\le I_2$ under the parameter choices in both theorems, which leads to contradiction. Therefore, we must have $\tau=T+1$ conditioned on $\cE$. Then, \eqref{eq:thm_up} implies
\begin{align*}
\frac{1}{T}\sum_{t=1}^{T-1}\norm{\nabla f(x_{t})}^2\le& I_1/T\le \epsilon^2,
\end{align*}
where the last inequality is due to Lemma~\ref{lem:calculations}.
\end{proof}


==> Sections/proof_vr.tex <==

\paragraph{Some definitions.}
Denote
\begin{align*}
\epsilon_t:=&m_t-\nabla f(x_t),
\end{align*}
From the update rule \eqref{eq:vr_adam}, we have
\begin{align}
	\epsilon_t = (1-\beta)\epsilon_{t-1}+W_t,\label{eq:vr_eps_recur}
\end{align}
where
\begin{align*}
	W_t:=& \nabla f(x_t,\xi_t)-\nabla f(x_t)-(1-\beta)\left(\nabla f(x_{t-1},\xi_t)- \nabla f(x_{t-1})\right).
\end{align*}
Compared with the ADAM part, the main difficulty here is that the momentum $m_t$ is not bounded every step. To overcome it, we impose such bound in the stopping time definition. In particular, given two constants $G$ and $E$, we define
\begin{align*}
\tau_1 :=& \min\{t\mid \norm{\nabla f(x_t)}>G\}\land (T+1),\\
\tau_2 :=& \min\{t\mid \norm{\epsilon_t}>E\}\land (T+1),\\
\tau:=& \min\{\tau_1,\tau_2\}.
\end{align*}
It is straight-forward to verify that $\tau_1,\tau_2,\tau$ are all stopping times. We will show that introducing this additional $\tau_2$ is fine because the probability that $\tau_2=\tau\le T$, i.e., the process stops due to $ \norm{\epsilon_t}>E$ for some $t$, is small.

With the new stopping time, we can bound the update at each step.
%\begin{lemma}
%		\label{lem:vr_bound_update}
%		If $t<\tau$, $\norm{x_{t+1}-x_t}\le 2\eta G/\lambda=:\eta D$.
%\end{lemma}
%\begin{remark}
%	When 
%\end{remark}
%
%We first start with a lemma that bounds the update $\norm{x_{t+1}-x_t}$ before time $\tau$.
%\begin{lemma}
%	\label{lem:vr_bound_update}
%	If $t<\tau$, $\norm{x_{t+1}-x_t}\le \eta (\norm{\nabla f(x_t)}+\norm{\epsilon_t})/\lambda\le \eta 2\eta G/\lambda$.
%\end{lemma}
%\begin{remark}\hfil
%\begin{itemize}
%	\item Note that Lemma~\ref{lem:vr_bound_update} does not give us an almostly sure constant bound as the RHS depends on $\epsilon_t$, which is not easy to bound. That is the reason we require $r=\infty$. We can only get the following bounds regardin $\epsilon_t$ which are unfortunately not enough
%	\begin{align*}
%	\E[\norm{\epsilon_1}^2]\le \cO(\epsilon),\quad \E[\norm{\epsilon_{\tau}}^2]\le \cO(\epsilon).
%	\end{align*}
%	\item We can also get a $G$-independent bound like $\norm{x_{t+1}-x_t}\le \eta (\lambda\sqrt{d}+\norm{\epsilon_t})/\lambda$ when $\betasq$ is small enough. However, even with this bound, we are still now able to do $1\le\rho<2$ because we can only use a loose way to bound $\norm{\epsilon_t}$ in the lower bound proof (see Lemma~\ref{lem:lower_vr}).
%\end{itemize}
%
%\end{remark}



\begin{lemma}
    \label{lem:vr_bound_update}
    Let $D :=\left\{
    \begin{array}{lr}
    \min\{2\sqrt{2d/\betasq},  2G/\lambda\}& \text{if } \sqrt{\betasq} \le \frac{\lambda}{2\sigma}, \\
    2 G/\lambda& \text{otherwise. } 
    \end{array}
    \right.$.
    If $E=\lambda D/6$ and $t<\tau$, $\norm{x_{t+1}-x_t}\le   \eta D$.
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lem:vr_bound_update}]
	First, irrespective of the value of $\betasq$, we always have
	\begin{align*}
		\norm{x_{t+1}-x_t}\le \eta\norm{m_t}/\lambda\le  \eta(\norm{\nabla f(x_t)}+\norm{\epsilon_t})/\lambda\le 2\eta G/\lambda.
	\end{align*}
	 If $\sqrt{\betasq}\le\frac{\lambda}{2\sigma}$, we have
	 \begin{align*}
	 \sqrt{\hv_t}+\lambda\succeq \sqrt{\betasq}\abs{\nabla f(x_t,\xi_t)}+\lambda\ge \sqrt{\betasq}\left(\nabla f(x_t)-\sigma\right)+\lambda\ge \sqrt{\betasq}\abs{\nabla f(x_t)}+\lambda/2.
	 \end{align*} 
	 Therefore,
	 \begin{align*}
	 	\abs{x_{t+1}-x_t}\preceq \frac{\eta \abs{m_t}}{\sqrt{\betasq}\abs{\nabla f(x_t)}+\lambda/2}\le \frac{\eta \left(\abs{\nabla f(x_t)}+\abs{\epsilon_t}\right) }{\sqrt{\betasq}\abs{\nabla f(x_t)}+\lambda/2}\le \eta\left(\frac{1}{\sqrt{\betasq}}+\frac{2\abs{\epsilon_t}}{\lambda} \right),
	 \end{align*}
	  which implies 
	  \begin{align*}
	  	 \norm{x_{t+1}-x_t}\le \sqrt{2}\eta\left(\sqrt{\frac{d}{\betasq}}+\frac{2\norm{\epsilon_t}}{\lambda}\right)\le \eta D.
	  \end{align*}
\end{proof}

Next, we bound $\norm{W_t}$ when $t\le\tau$.
\begin{lemma}
	\label{lem:vr_bound_Wt}
	If $t\le\tau$, $G\ge2\sigma$, and $\eta\le r/D$, 
	\begin{align*}
	\norm{W_t}\le \beta\sigma+\frac{4\eta(L_0+L_\rho G^\rho)}{\lambda}\left(\norm{\nabla f(x_{t-1})}+\norm{\epsilon_{t-1}}\right).
	\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lem:vr_bound_Wt}]
	By the definition of $W_t$, it is easy to verify that
	\begin{align*}
	W_t=\beta( \nabla f(x_t,\xi_t)-\nabla f(x_t)) + (1-\beta)\delta_t,
	\end{align*}
	where 
	\begin{align*}
	\delta_t= \nabla f(x_t,\xi_t)-\nabla f(x_{t-1},\xi_t)-\nabla f(x_t)+ \nabla f(x_{t-1}).
	\end{align*}
	By Assumption~\ref{ass:l0l1_vr}, we can bound
	\begin{align*}
	\norm{\delta_t}\le& \norm{\nabla f(x_t,\xi_t)-\nabla f(x_{t-1},\xi_t)}  +\norm{\nabla f(x_t) - \nabla f(x_{t-1})} \\
	\le&(L_0+L_\rho \norm{\nabla f(x_{t-1},\xi_t)}^\rho)\norm{x_t-x_{t-1}}+(L_0+L_\rho \norm{\nabla f(x_{t-1})}^\rho)\norm{x_t-x_{t-1}}\\
	\le & (L_0+L_\rho ({G+\sigma})^\rho)\norm{x_t-x_{t-1}}+(L_0+L_\rho G^\rho)\norm{x_t-x_{t-1}}\\
	\le& 4(L_0+L_\rho G^\rho)\norm{x_t-x_{t-1}}\\
	\le& \frac{4\eta(L_0+L_\rho G^\rho)}{\lambda}\left(\norm{\nabla f(x_{t-1})}+\norm{\epsilon_{t-1}}\right),
	\end{align*}
	where the second inequality uses Assumption~\ref{ass:l0l1_vr}; and the last inequality uses Lemma~\ref{lem:vr_bound_update}. Then, we have
	\begin{align*}
		\norm{W_t}\le \beta\sigma+\frac{4\eta(L_0+L_\rho G^\rho)}{\lambda}\left(\norm{\nabla f(x_{t-1})}+\norm{\epsilon_{t-1}}\right).
	\end{align*}
\end{proof}


The descent lemma still holds for VR ADAM.
\begin{lemma}
	\label{lem:descent_lemma_vr}
	If $t<\tau$, choosing $G\ge \sigma+\lambda$ and $\eta\le \min\{\frac{r}{D},\frac{\lambda}{6(L_0+L_\rho G^\rho)}\}$, we have
	\begin{align*}
	f(x_{t+1})-f(x_t) \le& -\frac{\eta}{4G}\norm{\nabla f(x_t)}^2 + \frac{\eta}{\lambda}\norm{\epsilon_t}^2.
	\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lem:descent_lemma_vr}]
Essentially the same as the proof of Lemma~\ref{lem:descent_lemma}. 
\end{proof}
\begin{lemma}
	\label{lem:moment_err_vr}
	If $G\ge \max\{2\sigma,2\lambda\}$ and $\eta\le \min\{\frac{r}{D}, \frac{\lambda^{3/2}}{32(L_0+L_\rho G^\rho)}\sqrt{\frac{\beta}{G}}\} $,
	\begin{align*}
	\E\left[\sum_{t=1}^{\tau-1} \frac{\beta}{2}\norm{\epsilon_t}^2-\frac{\lambda\beta}{16G}\norm{\nabla f(x_{t})}^2  \right]\le 4\sigma^2\beta^2 T  -\E[\norm{\epsilon_\tau}^2] .
	\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lem:moment_err_vr}]
	By Lemma~\ref{lem:vr_bound_Wt}, we have
	\begin{align*}
		\norm{W_t}^2\le& 2\sigma^2\beta^2+\frac{64\eta^2(L_0+L_\rho G^\rho)^2}{\lambda^2}\left(\norm{\nabla f(x_{t-1})}^2+\norm{\epsilon_{t-1}}^2\right)\\
		\le& 2\sigma^2\beta^2+\frac{\lambda\beta}{16G}\left(\norm{\nabla f(x_{t-1})}^2+\norm{\epsilon_{t-1}}^2\right),
	\end{align*}
	where in the second inequality we choose $\eta\le \frac{\lambda^{3/2}}{32(L_0+L_\rho G^\rho)}\sqrt{\frac{\beta}{G}}$.
	Therefore, noting that $\frac{\lambda\beta}{16G}\le \beta/2$, we have
	\begin{align*}
		\norm{\epsilon_t}^2\le (1-\beta/2)\norm{\epsilon_{t-1}}^2 + \frac{\lambda\beta}{16G}\norm{\nabla f(x_{t-1})}^2+2\sigma^2\beta^2+ (1-\beta)\innerpd{\epsilon_{t-1}}{W_t}.
	\end{align*}
	Summing over $2\le t\le \tau$ and re-arranging the terms, we get
	\begin{align*}
		\sum_{t=1}^{\tau-1} \frac{\beta}{2}\norm{\epsilon_t}^2-\frac{\lambda\beta}{16G}\norm{\nabla f(x_{t})}^2\le \norm{\epsilon_1}^2-\norm{\epsilon_\tau}^2+2\sigma^2\beta^2(\tau-1)+(1-\beta) \sum_{t=2}^\tau \innerpd{\epsilon_{t-1}}{W_t}.
	\end{align*}
	Taking expectations on both sides,  noting that
	\begin{align*}
		\E\left[ \sum_{t=2}^\tau \innerpd{\epsilon_{t-1}}{W_t}\right] =0
	\end{align*}
	by the optional stopping theorem (see Lemma~\ref{lem:optional_stoppping}), we have
	\begin{align*}
		\E\left[\sum_{t=1}^{\tau-1} \frac{\beta}{2}\norm{\epsilon_t}^2-\frac{\lambda\beta}{16G}\norm{\nabla f(x_{t})}^2  \right]\le 2\sigma^2\beta^2 T +\E[\norm{\epsilon_1}^2]-\E[\norm{\epsilon_\tau}^2]\le  4\sigma^2\beta^2 T  -\E[\norm{\epsilon_\tau}^2].
	\end{align*}
\end{proof}

\begin{lemma}
	\label{lem:upper_vr}
	Under the parameter choices in Theorem~\ref{thm:main_vr}, we have
	\begin{align*}
	\E\left[\sum_{t=1}^{\tau-1}\norm{\nabla f(x_{t})}^2\right]\le \frac{16G\Delta_0}{\eta},\quad \E[\norm{\epsilon_\tau}^2]\le  \frac{\lambda\Delta_0\beta}{\eta}.
	\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lem:upper_vr}]
	Combining Lemma~\ref{lem:descent_lemma_vr} and Lemma~\ref{lem:moment_err_vr}, it is easy to show
	\begin{align*}
	\E\left[\sum_{t=1}^{\tau-1}\norm{\nabla f(x_{t})}^2\right]\le \frac{8G\Delta_0}{\eta}+\frac{64G\sigma^2\beta T}{\lambda},\quad \E[\norm{\epsilon_\tau}^2]\le  4\sigma^2\beta^2 T+\frac{\lambda\Delta_0\beta}{2\eta}.
	\end{align*}
	Then by Lemma~\ref{lem:vr_parameters}, we complete the proof.
\end{proof}

%\begin{lemma}
%	\label{lem:bound_moment_near_tau}
%	Choosing $\beta\le \frac{4\eta(L_0+L_\rho G^\rho)}{\lambda}$, if $\tau-1/a\le t\le \tau$, where $a=8\eta(L_0+L_\rho G^\rho)/\lambda$, we have $\norm{\epsilon_t}\le 3(\norm{\epsilon_\tau}+G)$.
%\end{lemma}
%\begin{proof}[Proof of Lemma~\ref{lem:bound_moment_near_tau}]
%	%	By the update rule \eqref{eq:vr_adam} and triangle inequality, if $t\le\tau$,
%	%	\begin{align*}
%	%		\norm{m_{t}}\ge& (1-\beta)	\norm{m_{t-1}}-\beta\norm{\nabla f(x_t,\xi_t)}-\norm{\nabla f(x_t,\xi_t)-\nabla f(x_{t-1},\xi_t) }.
%	%	\end{align*}
%	%	It is not hard to show $\norm{\nabla f(x_t,\xi_t)}\le 2G$. Also note that
%	%	\begin{align*}
%	%		\norm{\nabla f(x_t,\xi_t)-\nabla f(x_{t-1},\xi_t) }\le \eta (L_0+L_{\rho}G^{\rho})\norm{m_{t-1}}
%	%	\end{align*}
%	%	Denoting $a=2\eta (L_0+L_{\rho}G^{\rho})\ge2\beta$, we have
%	%	\begin{align*}
%	%		\norm{m_{t-1}}\le\frac{\norm{m_t}}{1-a}+2\beta G.
%	%	\end{align*}
%	By Lemma~\ref{lem:vr_bound_Wt}, if $t\le\tau$, we have
%	\begin{align*}
%	\norm{W_t}\le \beta\sigma+\frac{4\eta(L_0+L_\rho G^\rho)}{\lambda}\left(G+\norm{\epsilon_{t-1}}\right)\le a G+a\norm{\epsilon_{t-1}}/2,
%	\end{align*}
%	where in the last inequality we choose $\beta\le \frac{4\eta(L_0+L_\rho G^\rho)}{\lambda}$. From \eqref{eq:vr_eps_recur}, we can bound
%	\begin{align*}
%	\norm{\epsilon_{t}}\ge (1-\beta)\norm{\epsilon_{t-1}}-\norm{W_t}\ge
%	(1-a)\norm{\epsilon_{t-1}}-a G.
%	\end{align*}
%	Then we can get for any $\tau-1/a\le t\le \tau$,
%	\begin{align*}
%	\norm{\epsilon_t}\le \frac{\norm{\epsilon_\tau}}{(1-a)^{\tau-t}} + aG\sum_{s=t}^{\tau-1}\frac{1}{(1-a)^{\tau-t}}\le \frac{\norm{\epsilon_\tau}}{(1-a)^{1/a}} + \frac{G}{(1-a)^{1/a}}\le 3(\norm{\epsilon_\tau}+G),
%	\end{align*}
%	where in the last inequality we use $(1-a)^{-1/a}\le e\le 3$.
%\end{proof}


\begin{lemma}
	\label{lem:lower_bound_vr} Suppose $G\ge 2\max\{\norm{\nabla f(x_1)},\sigma\}$ and $\eta\le\min\left\{\frac{r}{D},\frac{G}{4D(L_0+L_\rho G^\rho)}\right\} $. If  $\tau_1=\tau\le T$, i.e., there exists some time up to $T$ when the gradient norm is greater than $G$, the following inequality holds almost surely
	\begin{align*}
	\sum_{t=1}^{\tau-1} \norm{\nabla f(x_t)}^2> \frac{G^3}{16\eta D(L_0+L_\rho G^\rho)}.
	\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lem:lower_bound_vr}]
	Note that $\tau_1=\tau\le T$ implies $\norm{\nabla f(x_\tau)}>G$. The rest of proof is the same as that of Lemma~\ref{lem:lower_bound}.
\end{proof}
%
%\begin{lemma}
%	\label{lem:lower_vr} Under the parameter choices in Theorem~\ref{thm:main_vr},
%\begin{align*}
%		\E\left[\sum_{t=1}^{\tau-1}\norm{\nabla f(x_{t})}^2\right]\ge\frac{\lambda G^2}{32\eta (L_0+L_\rho G^{\rho})}\left(\Pro(\tau\le T)-\frac{\delta}{2}\right)+\Pro(\tau=T+1)\E\left[\sum_{t=1}^{\tau-1}\norm{\nabla f(x_{t})}^2\vert\Pro(\tau=T+1) \right].
%\end{align*}
%\end{lemma}
%\begin{proof}[Proof of Lemma~\ref{lem:lower_vr}]
%Let us first condition on the event $\tau\le T$. Let $a=8\eta(L_0+L_\rho G^\rho)/\lambda$. Then there are two cases
%\begin{enumerate}
%	\item If $\tau-\tau_{1/2}> 1/a$, then we directly have
%	\begin{align*}
%	G/2< a G (\tau-\tau_{1/2})/2.
%	\end{align*}
%	\item Otherwise if $\tau-\tau_{1/2}\le 1/a$, we have
%		\begin{align*}
%	G/2<& \norm{\nabla f(x_{\tau})-\nabla f(x_{\tau_{1/2})}}\\
%	\le &  \sum_{t=\tau_{1/2}}^{\tau-1} \norm{\nabla f(x_{t+1})-\nabla f(x_{t})} \\
%	\le &  \sum_{t=\tau_{1/2}}^{\tau-1} {\eta(L_0+L_\rho G^\rho)}\norm{x_{t+1}-x_t} \\
%	\le & \sum_{t=\tau_{1/2}}^{\tau-1} a(G+\norm{\epsilon_t})/8\\
%	\le & a G (\tau-\tau_{1/2})/2+\norm{\epsilon_\tau}/2.
%	\end{align*}
%	where the first inequality is due to $\norm{\nabla f(x_\tau)}> G$ and $\norm{\nabla f(x_{\tau_{1/2}})}\le G/2$ by the definition of $\tau$ and $\tau_{1/2}$; the third inequality is due to Assumption~\ref{ass:l0l1_vr}; the fourth inequality is due to Lemma~\ref{lem:vr_bound_update}; and the last inequality uses Lemma~\ref{lem:bound_moment_near_tau}.
%\end{enumerate}
%Combining the two cases, we have 
%\begin{align*}
%	G1_{\tau\le T}<aG(\tau-\tau_{1/2})1_{\tau\le T}+\norm{\epsilon_{\tau}}.
%\end{align*}
%Taking expectation, we have
%\begin{align*}
%	\E[(\tau-\tau_{1/2})1_{\tau\le T}]> \frac{1}{a}\Pro(\tau\le T)-\frac{1}{aG}\E[\norm{\epsilon_\tau}]\ge  \frac{1}{a}\left(\Pro(\tau\le T)-\frac{\delta}{4}\right),
%\end{align*}
%where in the last inequality we use the bound of $\E\left[\norm{\epsilon_\tau}^2 \right]$ in Lemma~\ref{lem:upper_vr}. Therefore
%\begin{align*}
%	\E\left[\sum_{t=1}^{\tau-1}\norm{\nabla f(x_{t})}^21_{\tau\le T}\right]\ge & 	\E\left[\sum_{t=\tau_{1/2}+1}^{\tau-1}\norm{\nabla f(x_{t})}^21_{\tau\le T}\right]\\
%	\ge& \left(\frac{G}{2}\right)^2\E[(\tau-\tau_{1/2}-1)1_{\tau\le T}]\\
%	\ge& \frac{\lambda G^2}{32\eta (L_0+L_\rho G^{\rho})}\left(\Pro(\tau\le T)-\frac{\delta}{4}\right)-\frac{G^2}{4}\\
%	\ge&\frac{\lambda G^2}{32\eta (L_0+L_\rho G^{\rho})}\left(\Pro(\tau\le T)-\frac{\delta}{2}\right).
%\end{align*}
%\end{proof}
\begin{proof}[Proof of Theorem~\ref{thm:main_vr}]
	Denote event $\cE:=\{\tau_1=\tau\le T\}$. Then by Lemma~\ref{lem:lower_bound_vr}, we can obtain
	\begin{align*}
	\E\left[\sum_{t=1}^{\tau-1}\norm{\nabla f(x_{t})}^2\right]\ge \Pro(\cE)\E\left[\sum_{t=1}^{\tau-1}\norm{\nabla f(x_{t})}^2\vert \cE \right]\ge \frac{G^3}{16\eta D(L_0+L_\rho G^\rho)}\cdot\Pro(\cE) .
	\end{align*}
Comparing with the upper bound in Lemma~\ref{lem:upper_vr}, we get
\begin{align*}
	\Pro(\cE)\le \frac{\delta}{4}.
\end{align*}
On the other hand, if $\tau_2=\tau\le T$, we know $\norm{\epsilon_\tau}>G$. However since $\E[\norm{\epsilon_\tau}^2]\le $ by Lemma~\ref{lem:upper_vr}, by Markov inequality, we have
\begin{align*}
	\Pro( \tau_2=\tau\le T) \le	\Pro( \norm{\epsilon_\tau}>G ) \le \frac{\lambda\Delta_0\beta}{\eta G^2}\le \frac{\delta}{4}.
\end{align*}
Therefore we have 
\begin{align*}
	\Pro(\tau\le T)\le \Pro( \tau_1=\tau\le T) + \Pro( \tau_2=\tau\le T) \le \frac{\delta}{2}.
\end{align*}
Also note that 
\begin{align*}
	\E\left[\sum_{t=1}^{\tau-1}\norm{\nabla f(x_{t})}^2\right]\ge \Pro(\tau=T+1)\E\left[\sum_{t=1}^{T}\norm{\nabla f(x_{t})}^2\vert \tau=T+1 \right]\ge \frac{1}{2}\E\left[\sum_{t=1}^{T}\norm{\nabla f(x_{t})}^2\vert \tau=T+1 \right].
\end{align*}
We can get
\begin{align*}
	\E\left[\frac{1}{T}\sum_{t=1}^{T}\norm{\nabla f(x_{t})}^2\vert \tau=T+1 \right]\le \frac{\delta\epsilon^2}{2}.
\end{align*}
By Markov inequality, letting $\cF:=\{\frac{1}{T}\sum_{t=1}^{T}\norm{\nabla f(x_{t})}^2>\epsilon^2\}$ be the non-convergence event, we have
\begin{align*}
	\Pro(\cF\vert \tau=T+1)\le \frac{\delta}{2}.
\end{align*}
Therefore,
\begin{align*}
	\Pro(\cF\cup \{\tau\le T\})\le \Pro(\tau\le T) + \Pro(\cF\vert \tau=T+1)\le \delta.
\end{align*}
\end{proof}
%\begin{proof}[Proof of Theorem~\ref{thm:main_vr}]
%	Comparing Lemma~\ref{lem:upper_vr} and Lemma~\ref{lem:lower_vr}, we can obtain that
%	\begin{align*}
%	\Pro(\tau\le T)\le \frac{\delta}{2}+\frac{512\Delta_0 P}{\lambda G}\le \frac{3}{4}\delta,
%	\end{align*}
%	and that
%	\begin{align*}
%	\E\left[\frac{1}{T}\sum_{t=1}^{T}\norm{\nabla f(x_{t})}^2\vert \tau=T+1 \right]\le \frac{32G\Delta_0}{\eta T}\le \frac{\delta\epsilon^2}{4}.
%	\end{align*}
%	Denote the event of non-convergence as $\cE=\{\frac{1}{T}\sum_{t=1}^{T}\norm{\nabla f(x_{t})}^2>\epsilon^2\}$. By Markov inequality, we have
%	\begin{align*}
%	\Pro(\cE\vert \tau=T+1)\le \frac{\delta}{4}.
%	\end{align*}
%	Then we have
%	\begin{align*}
%	\Pro(\cE\cup \tau\le T) \le  \Pro(\tau\le T)+\Pro(\cE\vert \tau=T+1)\le \delta,
%	\end{align*}
%	i.e., with probability at least $1-\delta$, we have both $\tau=T+1$ and $\frac{1}{T}\sum_{t=1}^{T}\norm{\nabla f(x_{t})}^2\le\epsilon^2$
%\end{proof}
